High Throughput Cryptocurrency Routing in Payment Channel Networks

Despite growing adoption of cryptocurrencies, making fast payments at scale remains a challenge. Payment channel networks (PCNs) such as the Lightning Network have emerged as a viable scaling solution. However, completing payments on PCNs is challenging: payments must be routed on paths with sufficient funds. As payments flow over a single channel (link) in the same direction, the channel eventually becomes depleted and cannot support further payments in that direction; hence, naive routing schemes like shortest-path routing can deplete key payment channels and paralyze the system. Today's PCNs also route payments atomically, worsening the problem. In this paper, we present Spider, a routing solution that "packetizes" transactions and uses a multi-path transport protocol to achieve high-throughput routing in PCNs. Packetization allows Spider to complete even large transactions on low-capacity payment channels over time, while the multi-path congestion control protocol ensures balanced utilization of channels and fairness across flows. Extensive simulations comparing Spider with state-of-the-art approaches shows that Spider requires less than 25% of the funds to successfully route over 95% of transactions on balanced traffic demands, and offloads 4x more transactions onto the PCN on imbalanced demands.

==> outline.tex <==
\section{Outline} \label{sec:outline}

\begin{outline}[enumerate]
\1 Intro
 \2 Packet vs Circuit
 \2 Imbalance

\1 Evaluation
	\2 SpeedyMurmurs, SilentWhispers
            \3 Randomness of partition - no consistent results
            \3 Not imbalance, efficiency aware
        \2 Deposit vs Throughput plot
\end{outline}


==> rebalancing.tex <==
We model on-chain payment channel rebalancing using variables $b_{(u,v)}$, which is the average rate at which payment channel $(u,v)$ receives new funds in the $u \rightarrow v$ direction via on-chain transactions. These funds would typically be withdrawn from another payment channel on which node $u$ is receiving more than it is sending. 
A positive rebalancing rate on some payment channels ($b_{(u,v)} > 0$) can improve network throughput beyond the upper bound presented in Proposition~\ref{prop: bounds}. 
However, rebalancing channels on chain is expensive for the routers both in time (due to transaction confirmation delays) and in transaction fees (paid to the miners). 
Thus routers may be unwilling to actively rebalance their payment channels unless the profit obtained from the higher utility is sufficient to offset the rebalancing costs.

We leave a full analysis of incentives for routers to future work, but we now consider a simple modification to the previous optimization problem to understand the impact of on-chain rebalancing:
\begin{align}
    \mathrm{maximize}  \qquad \sum_{i,j \in V} U\Big(\sum_{p\in\mathcal{P}_{i,j}} & x_p\Big) - \gamma \sum_{(u,v) \in E} b_{(u,v)} \label{eq: LP2} \\
\mathrm{s.t.} \qquad \qquad \qquad \sum_{p\in\mathcal{P}_{i,j}} x_p &\leq d_{i,j} \quad \forall i, j \in V  \\
\sum_{p\in\mathcal{P}:(u,v)\in p} x_p + \sum_{p\in\mathcal{P}:(v,u)\in p} x_p &\leq \frac{c_{(u,v)}}{\Delta} \quad \forall (u,v) \in E  \label{eq:capconstr2} \\
\sum_{p\in\mathcal{P}:(u,v)\in p} x_p - \sum_{p\in\mathcal{P}:(v,u)\in p} x_p  &\leq b_{(u,v)} \quad \forall (u,v) \in E  \label{eq:balconstr2} \\
x_p &\geq 0 \quad \forall p \in \mathcal{P} \\
b_{(u,v)} &\geq 0 \quad \forall (u,v) \in E \label{eq: LP last2}.  
\end{align}
The objective in the problem above consists of two terms. The first term is the total utility, which we would like to maximize. The second term is the ``cost'' of on-chain rebalancing at a total rate of $\sum_{(u,v) \in E} b_{(u,v)}$, which we would like to minimize. The parameter $\gamma$ dictates how we weight these two conflicting goals. We can interpret $\gamma$ as the increase in utility required to offset one unit of on-chain rebalancing rate. In practice, $\gamma$ would depend on a variety of factors, such as the ratio of blockchain transaction fees to routing fees and how the transaction fees are computed. For example, if blockchain transaction fees do not depend on transaction size, routers can reduce the cost of rebalancing by using larger transactions, thereby effectively reducing $\gamma$ in the above model. 

We now analyze how on-chain rebalancing impacts utility. Let $B \triangleq \sum_{(u,v) \in E} b_{(u,v)}$ be the total rate of on-chain rebalancing, and let's assume for simplicity that the payment channel capacities are unlimited.
For large $\gamma$, $B$ will be close to 0 in the optimal solution. From Proposition~\ref{prop: bounds}, we know that the maximum achievable throughput in this case is $\nu(C^*)$. On the other hand, for $\gamma \approx 0$, $B$ can become arbitrarily large. It is not difficult to see that the network throughput can satisfy all of the demand $\sum_{i,j} d_{i,j}$ in this case, provided that the links have sufficient capacity (i.e, if the constraints~\eqref{eq:capconstr2} are not tight). 
In general, as $\gamma$ decreases, the total utility and total rebalancing rate both increase in the optimal solution, until the utility reaches the maximum possible utility given the capacity constraints. 

We can show that the maximum achievable utility is a non-decreasing concave function of the total rebalancing rate. The argument is as follows. Let $t(B)$ be the maximum achievable utility for a bound $B$ on the total rebalancing rate. $t(B)$ is the solution of the following optimization problem:
\begin{align}
    \mathrm{maximize}  \qquad \sum_{i,j \in V} U\Big(\sum_{p\in\mathcal{P}_{i,j}} & x_p\Big)  \label{eq: LP3} \\
\mathrm{s.t.} \qquad \qquad \qquad \sum_{p\in\mathcal{P}_{i,j}} x_p &\leq d_{i,j} \quad \forall i, j \in V  \\
\sum_{p\in\mathcal{P}:(u,v)\in p} x_p + \sum_{p\in\mathcal{P}:(v,u)\in p} x_p &\leq \frac{c_{(u,v)}}{\Delta} \quad \forall (u,v) \in E  \label{eq:capconstr3} \\
\sum_{p\in\mathcal{P}:(u,v)\in p} x_p - \sum_{p\in\mathcal{P}:(v,u)\in p} x_p  &\leq b_{(u,v)} \quad \forall (u,v) \in E  \label{eq:balconstr3} \\
\sum_{(u,v) \in E} b_{(u,v)} &\leq B \\
x_p &\geq 0 \quad \forall p \in \mathcal{P} \\
b_{(u,v)} &\geq 0 \quad \forall (u,v) \in E \label{eq: LP last3}.  
\end{align}


$t(\cdot)$ is non-decreasing because the set of feasible solutions is non-decreasing in $B$. To see that $t(\cdot)$ is concave, consider arbitrary $B_1$ and $B_2$ and $\theta \in (0,1)$. Let $\{(x^1_p, b^1_{(u,v)}) : p \in \mathcal{P}, (u,v)\in E \}$ and $\{(x^2_p, b^2_{(u,v)}) : p \in \mathcal{P}, (u,v)\in E\}$ be the optimal solutions corresponding to $B_1$ and $B_2$. Then $\{(\theta x^1_p + (1-\theta) x^2_p, \theta b^1_{(u,v)} + (1-\theta) b^2_{(u,v)}) : p \in \mathcal{P}, (u,v)\in E \}$ is a feasible solution for bound $\theta B_1 + (1-\theta) B_2$, and it achieves a utility of $\theta t(B_1) + (1-\theta)t(B_2)$. Hence, $t(\theta B_1 + (1 - \theta) B_2) \geq \theta t(B_1) + (1-\theta) t(B_2)$, and $t(\cdot)$ is concave.



==> routing.tex <==
\section{Routing} 
\label{sec:routing}

%In order to successfully route transaction units through the network, paths having sufficient funds in their  payment channels must to be found. 
%Each time a transaction unit is sent along a path, the balances in payment channels along the path are offset by a small amount (equal to the size of the transaction unit). 

The key to effective routing in payment channel networks is to keep payment channels {\em balanced}. A payment channel becomes imbalanced when the transaction rate across it is higher in one direction than the other; the party making more payments eventually runs out of funds and cannot send further payments until it either receives funds from the other side, or it deposits new funds into the payment channel via an on-chain rebalancing transaction. Since on-chain transactions are expensive and slow, it is desirable to avoid them as much as possible. 

In this section, we take a first-principles approach to routing with rate-imbalance constraints. We first answer the question: What is the maximum achievable throughput in a payment channel network with and without on-chain rebalancing transactions? We use a fluid model of the network, wherein transactions between source, destination pairs are modeled as continuous flows, to show that the maximum achievable throughput depends on properties of a {\em payment graph} that captures how currency flows between network participants (\S\ref{sec: throughput}). We formulate optimization problems for routing with rate-imbalance constraints. These optimization problems generalize classical network utility maximization~\cite{num} formulations for routing and rate control in communication networks~\cite{kelly2005stability, eryilmaz2006joint}. We discuss how dual decomposition of these optimization problems leads naturally to decentralized algorithms for imbalance-aware routing in payment channel networks (\S\ref{sec: algorithm}).


\subsection{A Motivating Example}
\label{sec: motivating example}
To illustrate the importance of balanced routing, consider the 5-node payment-channel network shown in Fig.~\ref{fig:routing}.
Suppose sender, receiver pairs seek to transact at the rates shown in Fig.~\ref{fig:routing_pg}. For example, node 1 wishes to send at rate 1 to nodes 2 and 5, and node 2 wishes to send at rate 2 to node 4. 
%the following rates: $d_{1,2}=1, d_{1,5}=1, d_{2,4}=2, d_{3,2}=1, d_{3,5}=2, d_{4,1}=2, d_{4,3}=2, d_{5,3}=1$, where $d_{i,j}$ denotes the desired rate from $i$ to $j$. 
Fig.~\ref{fig:routing} shows two different routing strategies under these demands for a specific network topology.
In each case, we impose the constraint that the net rate in either direction of any edge must be equal to ensure that payment channels do not run out of funds.

Fig.~\ref{fig:routing_1} shows the result for shortest-path balanced routing, wherein senders route only along the shortest path to their receiver nodes.
 For example, node 4 routes a flow of rate 1 along the path $4\rightarrow 2 \rightarrow 1$ (shown in green). 
The maximum total rate ({\em throughput}) that can be sent by this routing scheme is 5 units; any rate assignment offering a higher throughput does not satisfy the rate-balance constraints. However, an alternate routing scheme of Fig.~\ref{fig:routing_2} in which senders do not necessarily send along the shortest paths achieves a higher throughput of 8 units.
Here, node 2 sends a flow of rate 1 along the path $2\rightarrow 3 \rightarrow 4$, while the shortest path is $2\rightarrow 4$. This enables nodes 3 and 4 to also send 1 unit of flow to nodes 2 and 3 respectively. 

\begin{figure}
    \centering
    \begin{tabular}{c c c}
        \begin{subfigure}{0.3\columnwidth}
            \centering
            \includegraphics[width=\columnwidth]{figures/payment_graph_1.pdf}\vspace*{-3mm}
            \subcaption{Payment graph}
\label{fig:routing_pg}
        \end{subfigure}&
         \begin{subfigure}{0.3\columnwidth}
            \centering
            \includegraphics[width=\columnwidth]{figures/routing_1.pdf}
            \subcaption{Shortest-path routing}
\label{fig:routing_1}
        \end{subfigure} &
        \begin{subfigure}{0.3\columnwidth}
            \centering
            \includegraphics[width=\columnwidth]{figures/routing_2.pdf}
            \subcaption{Optimal balanced routing}
\label{fig:routing_2}
        \end{subfigure}
    \end{tabular}
        \caption{Example illustrating balanced routing. (a) The payment graph shows the desired transaction rates between pairs of nodes. (b) and (c) The maximum transaction rate achievable with shortest-path routing and the optimal balanced routing schemes on the topology shown. Each dotted edge represents 1 unit of flow along the direction of the arrow. The colors indicate separate flows.}
 %\vspace*{-3mm}
\label{fig:routing}
\end{figure}



%and derive decentralized algorithms for solving these problems as well as simpler heuristic algorithms. Our work is inspired by prior work on optimization-based routing and rate control in communication networks~\cite{kelly2005stability, eryilmaz2006joint} and multipath transport protocols like MPTCP~\cite{wischik2011design}.


% Routing non-atomic transactions requires specifying a path for each of the individual \tus. 
%Our goal is to design a decentralized routing algorithm to maximize throughput while maintaining channel balance.
% such that the total amount of \tus~transferred through the payment channel network is maximized. 
%We first study a fluid model of the network (\S\ref{sec: fluid model}), wherein transactions between source, destination pairs are modeled as continuous flows. The model provides insights on the fundamental limits on throughput that can be achieved with balance constraints (\S\ref{sec: throughput}) and motivates our algorithms (\S\ref{sec: algorithm}).
% The magnitude of a flow essentially captures the average rate at which currency is transferred from the source to the destination corresponding to that flow. 
% Such a model allows us to formulate optimal routing as a linear program (LP), which in turn motivates \TheSystem 's decentralized algorithm. 
% The fluid model also helps provide insights on the fundamental limits of throughput that can be achieved. 
% We discuss the fluid model (\S\ref{sec: fluid model}) and bounds on flow (\S\ref{sec: throughput}) next, following which we present our algorithm (\S\ref{sec: algorithm}). 


\subsection{Limits on Throughput} 

\subsubsection{Fluid Model} 
\label{sec: fluid model}

Consider the payment channel network modeled as a graph $G(V, E)$, with routers $V$ and payment channels $E$. 
For any source, destination routers $i, j \in V$, let $d_{i,j} \geq 0$ denote the average rate at which transaction units have to be transferred from $i$ to $j$.
Let $c_e$ denote the total amount of funds in channel $e$, for $e\in E$, and $\Delta$ the average latency experienced by transactions due to network delays.
Lastly let $\mathcal{P}_{i, j}$ denote the set of paths from $i$ to $j$ in $G$, for $i,j\in V$. 
We include only `trails', i.e., paths without repeated edges, in $\mathcal{P}_{i,j}$. 

The network attempts to satisfy the demands $d_{i,j}$ by sending {\em flows} from source to destination routers.  
A flow is defined by a (path, value) tuple, where path denotes the route taken and value denotes the rate carried by the flow. 
Operationally this can be interpreted as routing transactions along the flow's path such that the average rate of currency transferred along the path equals the value of the flow. 

Valid flows must obey two main constraints. 
First, payment channels are limited in their capacity to process a large rate of transactions, because funds allocated to a transaction are unavailable to use for other transactions for some amount of time. Assume it takes $\Delta$ seconds on average for a transaction to reach its destination, get confirmed, and its hash lock key to reach the next payment channel on the upstream path. Then a payment channel with $c$ units of capacity can support, on an average, transactions of net value no more than $c/\Delta$ currency units per second. 
Second, to maintain balance the total flow along the two directions of a payment channel must be the same. 
If the flows are not balanced, the channel will eventually become unusable along one of the directions unless it is periodically rebalanced via on-chain transactions (we revisit this possibility below).

With these constraints, maximizing throughput in the fluid model is equivalent to finding flows of maximum total value and can be formulated as a Linear Program (LP):
\begin{align}
\mathrm{maximize}  \qquad \sum_{i,j \in V} \sum_{p\in\mathcal{P}_{i,j}} & x_p \label{eq: LP} \\
\mathrm{s.t.} \qquad \qquad \qquad \sum_{p\in\mathcal{P}_{i,j}} x_p &\leq d_{i,j} \quad \forall i, j \in V  \\
\sum_{p\in\mathcal{P}:(u,v)\in p} x_p + \sum_{p\in\mathcal{P}:(v,u)\in p} x_p &\leq \frac{c_{(u,v)}}{\Delta} \quad \forall (u,v) \in E  \label{eq:capconstr}\\
\sum_{p\in\mathcal{P}:(u,v)\in p} x_p - \sum_{p\in\mathcal{P}:(v,u)\in p} x_p  &\leq 0 \quad \forall (u,v) \in E  \label{eq:balconstr}\\
x_p &\geq 0 \quad \forall p \in \mathcal{P} \label{eq: LP last},  
\end{align}
Here, $x_p$ denotes the flow along path $p$ and $\mathcal{P} = \cup_{i,j\in V}\mathcal{P}_{i,j}$ is the set of all paths. The constraints in eq.~\eqref{eq:capconstr} reflect the capacity limits of payment channels, and the constraints in eq.~\eqref{eq:balconstr} enforce the balance requirement. 

%The parameter $B$ specifies the total amount of imbalance (across all links) that can be tolerated: $B=0$ corresponds to enforcing perfect balance. A larger value of $B$ permits more imbalance; as we discuss below, this can increase throughput but it also means that routers must make more on-chain transactions to rebalance payment channels.  

\subsubsection{Throughput under Perfect Balance} 
\label{sec: throughput}

Next, we show that the maximum throughput achievable under perfect balance is fundamentally restricted by the structure of  demand $[d]_{i,j}$ across nodes. Specifically the maximum throughput possible is equal to the largest amount of ``circulation'' contained in the demands, with higher throughputs possible only if payment channels are rebalanced via on chain transactions. 

\smallskip 
\noindent {\bf Payment graphs and circulation.}
Define a {\em payment graph} $H(V, E_H)$ as a weighted directed graph with nodes $V$ and edges $E_H$.
An edge $(i,j)\in E_H$ if $d_{i,j} > 0$ with $d_{i,j}$ also being the weight of that edge. 
Payment graphs do not depend on the network topology; they depend only on the pattern of payments between the network nodes. 
Payment graphs are useful for analyzing throughput because any flow imbalance across cuts of $H$ cannot be balanced by any routing scheme in the payment channel network $G$. 
Fig.~\ref{fig:payment_graph_1} shows the payment graph for the example discussed in \S\ref{sec: motivating example}. 

\begin{figure}
    \centering
    \begin{tabular}{c c c}
        \begin{subfigure}{0.3\columnwidth}
            \centering
            \includegraphics[width=\columnwidth]{figures/payment_graph_1.pdf}
            \subcaption{Payment graph}
\label{fig:payment_graph_1}
        \end{subfigure} &
        \begin{subfigure}{0.3\columnwidth}
            \centering
            \includegraphics[width=\columnwidth]{figures/payment_graph_2.pdf}
            \subcaption{Circulation}
\label{fig:payment_graph_2}
        \end{subfigure} &
        \begin{subfigure}{0.3\columnwidth}
            \centering
            \includegraphics[width=\columnwidth]{figures/payment_graph_3.pdf}
            \subcaption{DAG}
\label{fig:payment_graph_3}
        \end{subfigure}         
    \end{tabular}
        \caption{Payment graph corresponding to the demands in the example of Fig.~\ref{fig:routing}. It decomposes into a maximum circulation and DAG components as shown in (b) and (c).}
\label{fig:payment_graph}
%\vspace*{-3mm}
\end{figure}


We define the {\em circulation} graph of a payment graph $H$ as another directed weighted graph $C(V, E_C)$ with $E_C \subseteq E_H$,  $w_C(i, j) \leq w_H(i, j)$ for all $(i,j)\in E_C$, and
the total weight of incoming and outgoing edges being equal at any node. 
%  \\ $\sum_{u \in \Gamma_\mathrm{in}(v)} w_C(u, v) = \sum_{u' \in \Gamma_\mathrm{out}(v)} w_C(v, u')$, where $w_C(i,j)$ denotes the weight of edge $(i,j)$ in $C$; $\Gamma_\mathrm{in}(v), \Gamma_\mathrm{out}(v)$ denotes the set of incoming and outgoing neighbors of $v$ respectively in $C$; 
$w_C(i,j)$, $w_H(i,j)$ denote edge weight of edge $(i,j)$ in graphs $C$, $H$ respectively.
The circulation graph captures flows that form cycles in the payment graph. 
Letting $\sum_{(i,j) \in E_C} w_C(i,j)$ be the total {\em value} $\nu(C)$ of the circulation, there exists a circulation graph $C^*$ of maximum value for a given payment graph $H$. 
Maximum circulation graphs are not necessarily unique. 
A maximum circulation graph $C^*$ can be constructed by successively removing cycles of constant flow from $H$, and adding them to $C^*$.
The graph remaining after removing all cycles from $H$ is a weighted directed acyclic graph (DAG).
%, which we denote by $D^*$. 
Fig.~\ref{fig:payment_graph_2} and~\ref{fig:payment_graph_3} shows the decomposition of the payment graph of Fig.~\ref{fig:payment_graph_1} into circulation and DAG components.

%Then the following result holds; we omit the proof due to space constraints.
% have the foll now state our result and present a proof sketch. 
\begin{prop} \label{prop: bounds}
For a payment graph $H$ with a maximum circulation graph $C^*$, there exists a routing scheme that achieves a throughput of $\nu(C^*)$ with perfect balance (i.e., $B=0$) on a network with payment channels of unlimited capacity.
% and perfect balance (i.e., $B=0$). 
Conversely, no routing scheme can achieve a throughput greater than $\nu(C^*)$ with perfect balance on any network. 
\end{prop}
\begin{proof}
To see that a throughput of $\nu(C^*)$ is achievable, consider routing the circulation along any spanning tree $T$ of the payment network $G$. 
For any pair of nodes $i, j \in V$ there exists a unique path from $i$ to $j$ in $T$ through which $w_{C^*}(i,j)$ amount of flow can be routed. 
We claim that such a routing scheme is perfectly balanced on all the links. 
This is because for any partition $S, V\backslash S$ of $C^*$, the net flow going from $S$ to $V\backslash S$ is equal to the net flow going from $V\backslash S$ to $S$ in $C^*$. 
Since the flows along an edge $e$ of $T$ correspond precisely to the net flows across the partitions obtained by removing $e$ in $T$, it follows that the flows on $e$ are balanced as well. 

Next, to see that no balanced routing scheme can achieve a throughput greater than $\nu(C^*)$, assume the contrary and suppose there exists a balanced routing scheme $\mathtt{SCH}$ with a throughput greater than $\nu(C^*)$. 
Let $H_\mathtt{SCH} \subseteq H$ be a payment graph where the edges represent the portion of demand that is actually routed in $\mathtt{SCH}$. 
Since $\nu(H_\mathtt{SCH}) > \nu(C^*)$, $H_\mathtt{SCH}$ is not a circulation and there exists a partition $S, V\backslash S$ such that the net flow from $S$ to $V\backslash S$ is strictly greater than the net flow from $V\backslash S$ to $S$ in $H_\mathtt{SCH}$. 
However, the net flows routed by $\mathtt{SCH}$ across the same partition $S,V\backslash S$ in $G$ are balanced (by assumption) resulting in a contradiction. 
Thus we conclude there does not exist any balanced routing scheme that can achieve a throughput greater than $\nu(C^*)$. 
\end{proof}

Proposition~\ref{prop: bounds} shows that the maximum achievable throughput in a payment channel network with perfect balance can be less than 100\% if the demands for payments between nodes is not a circulation. For example, the routing presented in Fig.~\ref{fig:routing_2} corresponds precisely to routing the maximum circulation component of the payment graph (Fig.~\ref{fig:payment_graph_2}) and is hence optimal. Yet it is only able to route $8/12=75\%$ of the demands in the payment graph. The DAG component is not routable without violating the balance constraints. 

Using payment channels with higher capacity can mitigate problems caused by rate imbalance, but it cannot solve it fundamentally. A payment channel with more funds can sustain rate imbalance for a longer period of time, but it will eventually run out of funds if the rate imbalance persists. To remain usable in both directions, such a payment channel will have to be repeatedly rebalanced via on-chain transactions. In current implementations, rebalancing requires closing a payment channel and reopening a new one. However, two nodes can in principle use multiple smaller payment channels instead of a single large payment channel, so that they can rebalance them one at a time.

We next consider the possibility of such on-chain rebalancing and analyze its impact on throughput in the fluid model.

\subsubsection {Throughput with On-Chain Rebalancing}
%Routers in a payment channel network can rebalance their payment channels from time to time or as they become saturated (e.g., by moving funds between payment channels) via on-chain transactions. 
We model on-chain payment channel rebalancing using variables $b_{(u,v)}$, which is the average rate at which payment channel $(u,v)$ receives new funds in the $u \rightarrow v$ direction via on-chain transactions. These funds would typically be withdrawn from another payment channel on which node $u$ is receiving more than it is sending. 
A positive rebalancing rate on some payment channels ($b_{(u,v)} > 0$) can improve network throughput beyond the upper bound presented in Proposition~\ref{prop: bounds}. 
However, rebalancing channels on chain is expensive for the routers both in time (due to transaction confirmation delays) and in transaction fees (paid to the miners). 
Thus routers may be unwilling to actively rebalance their payment channels unless the profit obtained from the higher throughput is sufficient to offset the rebalancing costs.

We leave a full analysis of incentives for routers to future work, but we now consider a simple modification to the previous optimization problem to understand the impact of on-chain rebalancing:
\begin{align}
\mathrm{maximize}  \qquad \sum_{i,j \in V} \sum_{p\in\mathcal{P}_{i,j}} & x_p - \gamma \sum_{(u,v) \in E} b_{(u,v)} \label{eq: LP2} \\
\mathrm{s.t.} \qquad \qquad \qquad \sum_{p\in\mathcal{P}_{i,j}} x_p &\leq d_{i,j} \quad \forall i, j \in V  \\
\sum_{p\in\mathcal{P}:(u,v)\in p} x_p + \sum_{p\in\mathcal{P}:(v,u)\in p} x_p &\leq \frac{c_{(u,v)}}{\Delta} \quad \forall (u,v) \in E  \label{eq:capconstr2} \\
\sum_{p\in\mathcal{P}:(u,v)\in p} x_p - \sum_{p\in\mathcal{P}:(v,u)\in p} x_p  &\leq b_{(u,v)} \quad \forall (u,v) \in E  \label{eq:balconstr2} \\
x_p &\geq 0 \quad \forall p \in \mathcal{P} \\
b_{(u,v)} &\geq 0 \quad \forall (u,v) \in E \label{eq: LP last2}.  
\end{align}
The objective in the problem above consists of two terms. The first term is the total throughput, which we would like to maximize. The second term is the ``cost'' of on-chain rebalancing at a total rate of $\sum_{(u,v) \in E} b_{(u,v)}$, which we would like to minimize. The parameter $\gamma$ dictates how we weight these two conflicting goals. We can interpret $\gamma$ as the increase in throughput required to offset one unit of on-chain rebalancing rate. In practice, $\gamma$ would depend on a variety of factors, such as the ratio of blockchain transaction fees to routing fees and how the transaction fees are computed. For example, if blockchain transaction fees do not depend on transaction size, routers can reduce the cost of rebalancing by using larger transactions, thereby effectively reducing $\gamma$ in the above model. 

We now analyze how on-chain rebalancing impacts throughput. Let $B \triangleq \sum_{(u,v) \in E} b_{(u,v)}$ be the total rate of on-chain rebalancing, and let's assume for simplicity that the payment channel capacities are unlimited.
For large $\gamma$, $B$ will be close to 0 in the optimal solution. From Proposition~\ref{prop: bounds}, we know that the maximum achievable throughput in this case is $\nu(C^*)$. On the other hand, for $\gamma \approx 0$, $B$ can become arbitrarily large. It is not difficult to see that the network throughput can satisfy all of the demand $\sum_{i,j} d_{i,j}$ in this case, provided that the links have sufficient capacity (i.e, if the constraints~\eqref{eq:capconstr2} are not tight). 
In general, as $\gamma$ decreases, the total throughput and total rebalancing rate both increase in the optimal solution, until the throughput reaches the maximum possible throughput given the capacity constraints. 

We can show that the maximum achievable throughput is a non-decreasing concave function of the total rebalancing rate. The argument is as follows. Let $t(B)$ be the maximum achievable throughput for a bound $B$ on the total rebalancing rate. $t(B)$ is the solution of the following optimization problem:
\begin{align}
\mathrm{maximize}  \qquad \sum_{i,j \in V} \sum_{p\in\mathcal{P}_{i,j}} & x_p  \label{eq: LP3} \\
\mathrm{s.t.} \qquad \qquad \qquad \sum_{p\in\mathcal{P}_{i,j}} x_p &\leq d_{i,j} \quad \forall i, j \in V  \\
\sum_{p\in\mathcal{P}:(u,v)\in p} x_p + \sum_{p\in\mathcal{P}:(v,u)\in p} x_p &\leq \frac{c_{(u,v)}}{\Delta} \quad \forall (u,v) \in E  \label{eq:capconstr3} \\
\sum_{p\in\mathcal{P}:(u,v)\in p} x_p - \sum_{p\in\mathcal{P}:(v,u)\in p} x_p  &\leq b_{(u,v)} \quad \forall (u,v) \in E  \label{eq:balconstr3} \\
\sum_{(u,v) \in E} b_{(u,v)} &\leq B \\
x_p &\geq 0 \quad \forall p \in \mathcal{P} \\
b_{(u,v)} &\geq 0 \quad \forall (u,v) \in E \label{eq: LP last3}.  
\end{align}


$t(\cdot)$ is non-decreasing because the set of feasible solutions is non-decreasing in $B$. To see that $t(\cdot)$ is concave, consider arbitrary $B_1$ and $B_2$ and $\theta \in (0,1)$. Let $\{(x^1_p, b^1_{(u,v)}) : p \in \mathcal{P}, (u,v)\in E \}$ and $\{(x^2_p, b^2_{(u,v)}) : p \in \mathcal{P}, (u,v)\in E\}$ be the optimal solutions corresponding to $B_1$ and $B_2$. Then $\{(\theta x^1_p + (1-\theta) x^2_p, \theta b^1_{(u,v)} + (1-\theta) b^2_{(u,v)}) : p \in \mathcal{P}, (u,v)\in E \}$ is a feasible solution for bound $\theta B_1 + (1-\theta) B_2$, and it achieves a throughput of $\theta t(B_1) + (1-\theta)t(B_2)$. Hence, $t(\theta B_1 + (1 - \theta) B_2) \geq \theta t(B_1) + (1-\theta) t(B_2)$, and $t(\cdot)$ is concave.


\subsection{Algorithms} \label{sec: algorithm}
In this section, we derive decentralized algorithms for routing and rate control in payment channel networks based on the previous optimization problems. These algorithms follow naturally from a dual decomposition of the optimization problems and have the following basic structure. Each payment channel has a {\em price} in each direction. Routers locally update these prices based on both congestion and imbalance across payment channels. To select paths, end-hosts monitor the total price of different paths and choose the cheapest options. Using dual variables for prices is common in the utility-maximization-based rate control and routing literature (e.g., see~\cite{kelly2005stability}).
A key difference from prior work, however, is that in addition to price variables for link capacity constraints, we also have price variables for link balance constraints. 
This ensures that links with skewed balances have a high price and helps steer the routing towards rebalancing the payment channels. 


We focus on the optimization problem in eqs.~\eqref{eq: LP2}--\eqref{eq: LP last2} for the general case with on-chain rebalancing. The algorithm without on-chain rebalancing is a special case.

Consider the partial lagrangian:
\begin{align}
L(\mathbf{x}, \mathbf{b}, \mathbf{\lambda}, \mathbf{\mu}) = \sum_{i,j \in V} \sum_{p\in\mathcal{P}_{i,j}} x_p &- \gamma \sum_{(u,v) \in E} b_{(u,v)} \nonumber \\
&- \sum_{(u,v) \in E} \lambda_{(u,v)} \left[ \sum_{p\in\mathcal{P}:(u,v)\in p} x_p + \sum_{p\in\mathcal{P}:(v,u)\in p} x_p - \frac{c_{(u,v)}}{\Delta} \right] \nonumber \\
&- \sum_{(u,v) \in E} \mu_{(u,v)} \left[ \sum_{p\in\mathcal{P}:(u,v)\in p} x_p - \sum_{p\in\mathcal{P}:(v,u)\in p} x_p  - b_{(u,v)} \right],
\end{align}
where $\lambda_{(u,v)}$ and $\mu_{(u,v)}$ are lagrange variables corresponding to the capacity and rate-imbalance constraints in eq.~\eqref{eq:capconstr2} and eq.~\eqref{eq:balconstr2} respectively. The partial lagrangian can be rewritten as:
\begin{align}
L(\mathbf{x}, \mathbf{b}, \mathbf{\lambda}, \mathbf{\mu}) = &\sum_{i,j \in V} \left[ \sum_{p\in\mathcal{P}_{i,j}} x_p - \sum_{p\in\mathcal{P}_{i,j}} x_p \sum_{(u,v) \in p} \left( \lambda_{(u,v)} + \lambda_{(v,u)} + \mu_{(u,v)} - \mu_{(v,u)} \right) \right] \nonumber \\
& + \sum_{(u,v)\in E} \left( \mu_{(u,v)} - \gamma \right) b_{(u,v)} + \sum_{(u,v)\in E} \lambda_{(u,v)}\frac{c_{(u,v)}}{\Delta}.
\end{align}
Define $z_{(u,v)} \triangleq \lambda_{(u,v)} + \lambda_{(v,u)} + \mu_{(u,v)} - \mu_{(v,u)}$ to be the price for edge $(u,v) \in E$, and $z_p \triangleq \sum_{(u,v)\in p} z_{(u,v)}$ to be price for path $p\in \mathcal{P}$. The important fact about the above partial lagrangian is that it decomposes into separate terms for the rate variables of each source/destination pair $\{x_p: p \in \mathcal{P}_{i,j}\}$, and the rebalancing rate of each edge $b_{(u,v)}$. This suggests the following primal-dual algorithm for solving the optimization problem in eqs.~\eqref{eq: LP2}--\eqref{eq: LP last2}:
\begin{itemize}
    \item {\bf Primal step.} Given the edge prices $z_{(u,v)}(t)$ at time $t$, for each source/destination pair $(i,j)$, update the sending rate on paths $p \in \mathcal{P}_{(i,j)}$ as follows:
    \begin{align}
    x_p(t) &= x_p(t-1) + \alpha \left(1 - z_p(t) \right), \nonumber \\ 
    x_p(t) &= \mathrm{Proj}_{\mathcal{X}_{i,j}}(x_p(t)), \label{eqn:primal_xp}
    \end{align}
    where $\mathrm{Proj}_{\mathcal{X}_{i,j}}(\cdot)$ stands for projection onto the convex set $\mathcal{X}_{i,j} = \{x_p~\mathrm{for}~p\in \mathcal{P}_{i,j} | x_p \geq 0, \sum_{p\in\mathcal{P}_{i,j}} x_p \leq d_{i,j} \}$. 

    At time $t$, each edge $(u,v)$ also updates its on-chain rebalancing rate according to:
    \begin{equation}
    b_{(u,v)}(t) = \left[ b_{(u,v)}(t-1) + \beta \left( \mu_{(u,v)}(t) - \gamma \right) \right]_+, \label{eqn:primal_b}
    \end{equation}
    where $\left[ \cdot \right]_+\triangleq max(\cdot,0)$. 

    \item {\bf Dual step.} In the dual step, the routers update the edge prices based on capacity and imbalance  constraints at the payment channels. Specifically, each edge performs the following updates independently:
    \begin{align}
    \lambda_{(u,v)}(t+1) &= \left[  \lambda_{(u,v)}(t) + \eta \left( \sum_{p\in\mathcal{P}:(u,v)\in p} x_p(t) + \sum_{p\in\mathcal{P}:(v,u)\in p} x_p(t) - \frac{c_{(u,v)}}{\Delta} \right) \right]_+, \label{eqn:cap_price} \\ 
    \mu_{(u,v)}(t+1) &= \left[  \mu_{(u,v)}(t) + \kappa \left( \sum_{p\in\mathcal{P}:(u,v)\in p} x_p(t) - \sum_{p\in\mathcal{P}:(v,u)\in p} x_p(t)  - b_{(u,v)} \right) \right]_+. \label{eqn:imb_price}
    \end{align}

\end{itemize}

The parameters $\alpha, \beta, \eta, \kappa$ are positive ``step size'' constants that determine the speed of the dynamics. Using standard arguments, it can be shown that for sufficiently small step sizes, the above algorithm converges to the optimal solution of the optimization problem in eqs.~\eqref{eq: LP2}--\eqref{eq: LP last2}.

The algorithm has the following intuitive interpretation: $\lambda_{(u,v)}$ and $\mu_{(u,v)}$ are prices that vary due to capacity constraints and imbalance at the payment channels. In eq.~\eqref{eqn:cap_price}, $\lambda_{(u,v)}$ increases if the net rate across the payment channel $(u,v)$ (in both directions) exceeds its capacity, and it decreases down to zero if there is excess capacity. Similarly, in eq.~\eqref{eqn:imb_price}, $\mu_{(u,v)}$ increases if the rate in the $(u,v)$ direction exceeds the rate in the $(v,u)$ direction by more than $b_{(u,v)}$, the rate at which funds are deposited for edge $(u,v)$ on chain. As these prices vary, each source/destination pair reacts by changing the sending rate on its paths according to eq.~\eqref{eqn:primal_xp}. The effect is to reduce the rate on expensive paths and increase it on cheap paths. Simultaneously, each edge also adapts its on-chain rebalancing rate based on eq.~\eqref{eqn:primal_b}. If $\mu_{(u,v)} > \gamma$, the price charged for imbalance is higher than the cost of on-chain rebalancing per unit rate. Hence the edge increases its on-chain rebalancing rate $b_{(u,v)}$; otherwise it decreases its throughput.
Finally, we note that in the absence of any on-chain rebalancing, the algorithm can be simplified by setting $b_{(u,v)} = 0$ for all edges $(u,v)$.

We remark that the objective of our optimization problem in eq.~\eqref{eq: LP} can be modified to also ensure fairness in routing, by associating an appropriate utility function with each sender-receiver pair~\cite{kelly1998rate}. 
A decentralized algorithm for such a case may be derived analogously as our proposed solution. 
% Since the optimal solution to the LP may assign zero flows to some demands, we consider a variant of the optimization problem that makes flow assignments fairly. 
% To obtain proportional-fairness we modify the LP's objective to maximize $\sum_{i,j}\log (\sum_{p\in\mathcal{P}_{i,j}} x_p)$ without modifying any of the constraints. 
% Alternative metrics for fairness can also be used. 

% Now, let $y^1_{i,j}, y^2_e, y^3_e$ for $i,j \in V, e\in E$ denote price variables corresponding to the total demand, capacity and balance constraints respectively.
% With a slight abuse of notation, let $y^{(\cdot)}_p$ be the sum total of edge price $y^{(\cdot)}_e$ along path $p$. 
% Similarly let $x_e$ be the total flow across edge $e$, and $x_{i,j}$ the total flow of demand $i,j$. 
% At each time round $t$, the payment channel prices are updated as $y^1_{i,j}(t+1) = y^1_{i,j}(t) + \eta (d_{i,j} - x_{i,j}(t))~\forall i,j\in V$, $y^2_{u,v}(t+1) = y^2_{u,v}(t) + \eta (c_{u,v} - x_{u,v}(t))~\forall (u,v) \in E $, $y^3_{u,v}(t+1) = y^3_{u,v}(t) + \eta (x_{v, u}(t) - x_{u,v}(t))~\forall (u,v) \in E$ where $\eta$ is a small step-size parameter. 
% Whereas the flow along the paths for each $i,j\in V$ are updated as $x_p(t+1) = 1/(\min_{p\in\mathcal{P}_{i,j}}(y^1_{i,j}(t) + y^2_p(t) + y^3_p(t) - y^3_{-p}(t)))$ for $p = \mathrm{argmin}_{p\in\mathcal{P}_{i,j}} (y^1_{i,j}(t) + y^2_p(t) + y^3_p(t) - y^3_{-p}(t))$, and $x_p(t+1) = 0$ otherwise. 
% Here for a path $p$, $-p$ refers to the path obtained by traversing $p$ in reverse order. 

\subsubsection{Practical considerations}

In practice, routers have to dynamically estimate the rate over their payment channels from the transactions that they encounter. 
The source nodes, whenever they have to send transactions, query for the path prices, and adapt the rate on each path based on these prices. 
This rate adaptation can occur in different ways depending on the implementation. For example, in an implementation where source nodes use only one path for routing each transaction, they can select these paths such that the frequency of usage of different paths over time is roughly proportional to the optimal flow rate along the paths. In the next section, we describe a design that allows more fine-grained rate control by splitting transactions into small units than can be transmitted on different paths.

A typical challenge with such iterative algorithms for adjusting path prices and sending rates is slow convergence. An algorithm that is slow to converge may not be able to adapt the routing to changes in the transaction arrival pattern. If the transaction arrival patterns change frequently, this may result in a perpetually suboptimal routing.

Therefore in practice it may be beneficial to also consider simpler approaches to balancing transactions across different paths that can converge quickly. One such approach is for sources to independently try to minimize imbalance on their paths by always sending on paths with the largest available capacity, much like ``waterfilling'' algorithms for max-min fairness. A source measures the available capacity on a set of paths to the destination. It then first transmits on the path with highest capacity until its capacity is the same as the second-highest-capacity path; then it transmits on both of these paths until they reach the capacity of the third highest-capacity-path, and so on. 

For both types of algorithms, practical implementations would restrict the set of paths considered between each source and destination, so that the overhead of probing the path conditions is not too high. There are a variety of possible strategies of selecting these paths, e.g., the $K$ shortest paths or the $K$ highest-capacity paths between every source/destination pair. We leave an investigation of the best way to select the paths to future work.

% for practicality. 
% The simplified heuristic, called the `waterfilling' heuristic, measures the available capacity on paths and routes on the path having the most available capacity (\S\ref{sec:eval-setup}).

% according to the total volume and imbalance of flows across the channel. 
%Users then route \tus~on paths having the cheapest price. 
%Using dual variables for routing is common, and can be found in the works [ ... ]our approach is similar to~\cite{kelly2005stability}.

 




